On the Disambiguation of Weighted Automata

We present a disambiguation algorithm for weighted automata. The algorithm admits two main stages: a pre-disambiguation stage followed by a transition removal stage. We give a detailed description of the algorithm and the proof of its correctness. The algorithm is not applicable to all weighted automata but we prove sufficient conditions for its applicability in the case of the tropical semiring by introducing the *weak twins property*. In particular, the algorithm can be used with all acyclic weighted automata, relevant to applications. While disambiguation can sometimes be achieved using determinization, our disambiguation algorithm in some cases can return a result that is exponentially smaller than any equivalent deterministic automaton. We also present some empirical evidence of the space benefits of disambiguation over determinization in speech recognition and machine translation applications.

==> alt.tex <==
\subsection{Alternative \Dis\ algorithm}

Here, we discuss another technique for the removal of transitions. To
determine the co-reachability of the states of a pre-disambiguated
automaton $A'$, we can compute the intersection $B = A' \cap A'$, the
accessible of states $((q, s), (q', s'))$ of $B$ determine exactly the
pairs of co-reachable states. It is in fact not necessary to keep the
transitions of $B$ in this computation since only the states are
needed. This suggests a transition removal process based on the
discovery of new pairs of such co-reachable states $((q, s), (q',
s'))$. 

Consider an arbitrary total order $<$ over the states of $A$.  Fix $a
\in \Sigma$ and a state $(q_0, s_0)$ of $A'$. In the process of
transition removal, some states are marked as \emph{needed} and that
property is maintained. The outgoing transition labeled with $a$ of
these states is then never removed.  For any co-reachable pair $((q,
s), (q', s'))$ with $(q, s)$ and $(q', s')$ both admitting a
transition labeled with $a$ to the same state $(q_0, s_0)$, if $q >
q'$ the state $(q, s)$ is marked as needed and the outgoing transition
of $(q', s')$ labeled with $a$ to $(q_0, s_0)$ is removed; if $q' >
q$, then $(q', s')$ is marked as needed and the outgoing transition of
$(q, s)$ labeled with $a$ to $(q_0, s_0)$ is removed. We will refer by
\emph{processing of the pairs} admitting a transition labeled with $a$
to $(q_0, s_0)$ the transition removal process just described. Note
that for a pair of distinct co-reachable states $((q, s), (q', s'))$
by some string $x$, we must have $q \neq q'$ since $s = s(q, x)$ and
$s' = s(q', x)$.

The \emph{processing of final pairs} is defined in a similar way: for any
co-reachable pair $((q, s), (q', s'))$ with $(q, s)$ and $(q', s')$
both final, if $q > q'$, state $(q, s)$ is marked as needed for
finality and state $(q', s')$ made non-final and vice-versa if $q' >
q$. 

\begin{lemma}
\label{lemma:12}
Let $A' = (Q', I', F', E', \rho')$ be the finite automaton returned by
the \predis\ of the weighted automaton $A = (Q, I, F, E, \rho)$.  Let
$(q_0, s_0)$ be a state of $A'$ and $a \in \Sigma$, then, the
automaton $A''$ resulting from processing the pairs labeled with $a$
to $(q_0, s_0)$ accepts the same strings as $A'$. Similarly, the
processing of final pairs of $A'$ does not affect the set of strings
accepted by $A'$.
\end{lemma}

\begin{proof}
  Fix $a \in \Sigma$ and state $(q_0, s_0)$ of $A'$. Assume that
  before the comparison of the pair of distinct co-reachable states
  $((q_2, s_2), (q_1, s_1))$ with $q_2 > q_1$, $A'$ is equivalent to
  $A$.  Assume that after comparison, $A'$ is not equivalent to
  $A$. This implies that the transition from $(q_1, s_1)$ is removed,
  otherwise $A'$ remains unchanged.  The removal occurs because $(q_2,
  s_2)$ and $(q_1, s_1)$ are both in $\delta(I', x_1)$ for some $x_1
  \in \Sigma^*$. $(q_1, s_1)$ must be reachable by some string $x_2
  \neq x_1$ that does not reach $(q_2, s_2)$, otherwise after removal
  $A$ and $A'$ remain equivalent.  By Lemma~\ref{lemma:1}, for any
  such string $x_2$, there exists $(q_2, s'_2)$ reachable by $x_2$ and
  admitting a transition labeled with $a$ to $(q_0, s_0)$. That
  $a$-transition must have been removed, otherwise $A$ and $A'$ would
  still be equivalent. If it has been removed, there must have been a
  comparison of a distinct pair $((q_3, s_3), (q_2, s'_2))$ with $q_3
  > q_2$ and $(q_3, s_3)$ and $(q_2, s'_2)$ both reachable by $x_2$
  causing that removal. $(q_2, s'_2)$ must be reachable by some string
  $x_3 \neq x_2$, otherwise after that removal $A'$ and $A$ remain
  equivalent. Proceeding in this way, we can construct an infinite
  sequence of states $(q_1, s_1), (q_2, s_2), \ldots, (q_k, s_k),
  \ldots$ with $q_1 > q_2 > \cdots > q_k > \cdots$ and $q_{i + 1} \neq
  q_i$ for all $i \geq 1$. This contradicts the finiteness of the
  number of states after pre-disambiguation and shows that the
  assumption that $A'$ is not equivalent to $A$ after the comparison
  $((q_2, s_2), (q_1, s_1))$ cannot hold. The reasoning is the same
  after processing of final pairs.\qed
\end{proof}


